Client/Server Based Online Environment for Manual Segmentation of Medical Images

Segmentation is a key step in analyzing and processing medical images. Due to the low fault tolerance in medical imaging, manual segmentation remains the de facto standard in this domain. Besides, efforts to automate the segmentation process often rely on large amounts of manually labeled data. While existing software supporting manual segmentation is rich in features and delivers accurate results, the necessary time to set it up and get comfortable using it can pose a hurdle for the collection of large datasets. This work introduces a client/server based online environment, referred to as Studierfenster (studierfenster.at), that can be used to perform manual segmentations directly in a web browser. The aim of providing this functionality in the form of a web application is to ease the collection of ground truth segmentation datasets. Providing a tool that is quickly accessible and usable on a broad range of devices, offers the potential to accelerate this process. The manual segmentation workflow of Studierfenster consists of dragging and dropping the input file into the browser window and slice-by-slice outlining the object under consideration. The final segmentation can then be exported as a file storing its contours and as a binary segmentation mask. In order to evaluate the usability of Studierfenster, a user study was performed. The user study resulted in a mean of 6.3 out of 7.0 possible points given by users, when asked about their overall impression of the tool. The evaluation also provides insights into the results achievable with the tool in practice, by presenting two ground truth segmentations performed by physicians.

==> Makefile <==
# GNU Makefile for LaTeX.
# (c) 2005 Georg Zotti, Institute of Computer Graphics, TU Vienna
# <gzotti(at)cg.tuwien.ac.at>

# Replace this by the name of your main .tex file (without the .tex)
BASENAME=cescg_09

# Add all your sourcefile names here. If you only have one .tex file, leave it as is. 
SOURCES = $(BASENAME).tex
# Here come the .bib files. If you don't use BibTeX, delete all entries here!
BIBFILES=cescg_09.bib

# If you use ``classic'' latex: Add image names (*.eps) which get automatically created from jpg, tiff, etc. 
# THESE WILL BE DELETED with "make pristine"!
TMP_EPS=

# If you use pdflatex: Add image names (*.pdf) which get automatically created from eps etc. 
# THESE WILL BE DELETED with "make pristine"!
TMP_PDF=



.SUFFIXES:
.SUFFIXES: .dtx .tex .aux .log .lot .lof .toc .glo .gls .ilg .dvi .ps .pdf .eps .jpg .png .tiff
.PHONY:  ins eps dvi ps pdf show clean pristine classdoc

help:
	@echo "Use targets: dvi, ps, pdf create documents"
	@echo "             show         use xdvi to show dvi"
	@echo "             clean        delete intermediate files, but leave auto-converted EPS images"
	@echo "             pristine     delete all intermediate and formatted files"
	@echo "             classdoc     make cescg.dvi"

dvi : $(BASENAME).dvi
ps  : $(BASENAME).ps
pdf : $(BASENAME).pdf

$(BASENAME).dvi:  $(SOURCES) $(TMP_EPS) $(BASENAME).bbl 
#	latex $(BASENAME).tex
#	bibtex $(BASENAME)
	latex $(BASENAME).tex
	latex $(BASENAME).tex

$(BASENAME).ps: $(BASENAME).dvi
	dvips  -Ppdf -ta4 -G0 -o $(BASENAME).ps $(BASENAME).dvi 

# The first variant is fine for GhostScript 7.x, the second is for GhostScript 8.x!
#$(BASENAME).pdf: $(BASENAME).ps
#	ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
#               -dSubsetFonts=true -dEmbedAllFonts=true \
#               -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
#               -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
#               -dMonoImageFilter=/FlateEncode $(BASENAME).ps $(BASENAME).pdf
#	ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3  \
#               -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
#               -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
#               -dMonoImageFilter=/FlateEncode $(BASENAME).ps $(BASENAME).pdf

eps: $(TMP_EPS)

# If you use pdflatex, you may acivate these lines and delete the lines above 
pdf $(BASENAME).pdf: $(BASENAME).bbl $(SOURCES) $(TMP_PDF)
	pdflatex $(BASENAME).tex
	bibtex $(BASENAME)
	pdflatex $(BASENAME).tex
	pdflatex $(BASENAME).tex

show: $(BASENAME).dvi
	xdvi -s 7 $(BASENAME).dvi &
# intermediate steps

$(BASENAME).bbl: $(BIBFILES) $(BASENAME).aux $(SOURCES)
	bibtex $(BASENAME)

$(BASENAME).aux: $(TMP_EPS) $(SOURCES)
	latex $(BASENAME).tex

# removing intermediate files or also the printable documents

clean:
	rm -f *~ *.aux *.bbl *.blg *.idx *.ilg *.ind *.log *.toc *.glo *.gls *.ilg 

pristine: clean
	rm -f $(BASENAME).pdf $(BASENAME).ps $(BASENAME).dvi *.tfm *pk $(TMP_EPS) $(TMP_PDF) 

.tiff.eps:
	convert $< eps:$@

.jpg.eps:
	convert $< eps:$@

.png.eps:
	convert $< eps:$@

.eps.pdf:
	cat $< | tr \\015 \\012 | epstopdf --filter > $@

classdoc: cescg.dtx
	latex cescg.dtx
	makeindex -s gglo.ist -o cescg.gls cescg.glo
	latex cescg.dtx

ins: cescg.dtx
	latex cescg.ins

cescg.cls cescgsmpl.tex example.eps smplbib.bib: ins

